Information Content in Neuronal Calcium Spike Trains: Entropy Rate Estimation based on Empirical Probabilities

Quantification of information content and its temporal variation in intracellular calcium spike trains in neurons helps one understand functions such as memory, learning, and cognition. Such quantification could also reveal pathological signaling perturbation that potentially leads to devastating neurodegenerative conditions including Parkinson's, Alzheimer's, and Huntington's diseases. Accordingly, estimation of entropy rate, an information-theoretic measure of information content, assumes primary significance. However, such estimation in the present context is challenging because, while entropy rate is traditionally defined asymptotically for long blocks under the assumption of stationarity, neurons are known to encode information in short intervals and the associated spike trains often exhibit nonstationarity. Against this backdrop, we propose an entropy rate estimator based on empirical probabilities that operates within windows, short enough to ensure approximate stationarity. Specifically, our estimator, parameterized by the length of encoding contexts, attempts to model the underlying memory structures in neuronal spike trains. In an example Markov process, we compared the performance of the proposed method with that of versions of the Lempel-Ziv algorithm as well as with that of a certain stationary distribution method and found the former to exhibit higher accuracy levels and faster convergence. Also, in experimentally recorded calcium responses of four hippocampal neurons, the proposed method showed faster convergence. Significantly, our technique detected structural heterogeneity in the underlying process memory in the responses of the aforementioned neurons. We believe that the proposed method facilitates large-scale studies of such heterogeneity, which could in turn identify signatures of various diseases in terms of entropy rate estimates.

==> figures/figure1/fig1.tex <==
\begin{figure}[ht!] 
     \begin{center}
\begin{tabular}{cc} 
        \subfigure[ ]{%
           \includegraphics[width=0.5\columnwidth]{figures/figure1/fig_1a_left.eps}
            %\includegraphics[width=\columnwidth]{figures/figure5_new/fig_5a.eps}

\label{fig:1a} 
        } 
         \subfigure[]{%
         \includegraphics[width=0.5\columnwidth]{figures/figure1/fig_1b.eps}
           \label{fig:1b}
        }
\end{tabular}
\end{center} 
 \caption{Intracellular calcium imaging in single neuron and associated dendrites and axon. (a) Representative image of neuron; (b) Time course of nomalized Fluo-4 intensity ($\Delta F/F_0$, as explained in Section \ref{spikeTrain}) in soma region (black), axon (blue) and dendrites (red). Scale bar = 20 $\mu$m.}
   \label{fig:1}
\end{figure}

%\begin{figure}[t!]
%\centering
%\includegraphics[width=\columnwidth]{figures/figure1/fig_1.eps}
%\caption{Single cell imaging: Intracellular calcium imaging in single neuron and associated dendrites and axon. (a) Representative image of a single neuron (b) Time course of Fluo-4 intensity in soma region, dendrite and axon (Green-soma, Blue- axon, red-dendrites).}
%\label{fig:1}
%\end{figure}

==> figures/figure2/fig2.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.8\columnwidth]{figures/figure2/fig2.eps} \vspace{0.3cm}
\caption{Multicell time lapse imaging of intracellular calcium in hippocampal neuron population: (a) Representative time lapse images of a neuronal network; (b) Time course of normalized Fluo-4 intensity ($\Delta F/F_0$, as explained in Section \ref{spikeTrain})  in 6 representative cells of the population. Scale bar = 20 $\mu$m.}
\label{fig:2}
\end{figure}


==> figures/figure3/fig3.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/figure3/fig3.eps}
\caption{Connectivity map and calcium spiking: (a) Two connected neurons; (b) Time course of normalized Fluo-4 intensity ($\Delta F/F_0$, as explained in Section \ref{spikeTrain}) in dendrites (red), soma (black) and axon (blue) for each neuron. Scale bar = 20 $\mu$m.}
\label{fig:3}
\end{figure}

==> figures/figure4/fig4.tex <==
\begin{figure}[t!] 
     \begin{center}
\begin{tabular}{cc} %\vspace{-0.2cm}
        \subfigure[ ]{%
            \includegraphics[width=\columnwidth]{figures/figure4/f1_edited_1.eps}
                \label{fig:4a}
\label{fig:first}
        } \\ %\vspace{-0.38cm}
         \subfigure[ ]{%
           \includegraphics[width=\columnwidth]{figures/figure4/f2_edited_1.eps}
           \label{fig:4b}
        }\\ 
        \subfigure[ ]{%
         \includegraphics[width=\columnwidth]{figures/figure4/f3_edited_1.eps}
           \label{fig:4c}
        }%
\end{tabular}
\end{center} \vspace{0.35cm}
    \caption{Spike train inference: (a) Time course of fluorescence intensity; (b) Spike probability estimation using fast nonnegative deconvolution ($P_{th}= 0.4828$); (c) Spike train along with amplitude.}
   \label{fig:4}
\end{figure}

==> figures/figure5_1/fig5.tex <==
\begin{figure}[t!] 
\begin{tabular}{c}
        \subfigure[]{
            \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5a_left.eps}
                  \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5a_right.eps}
       \label{fig:5a}
        }\\ \vspace{-0.1cm}
        \subfigure[]{%
         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5b_left.eps}
          \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5b_right.eps}
           \label{fig:5b}
       }\\ \vspace{-0.3cm}
 \subfigure[]{%
         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5c_left.eps}
          \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5c_right.eps}
           \label{fig:5c}
}\\
 \subfigure[]{%
         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5d_left.eps}
\includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5d_right.eps}
           \label{fig:5d} 
}

\end{tabular} \vspace{0.5cm}
\caption{Calcium oscillation: (left panels) Calcium responses; (right panels) Raster plots of 
soma (black), dendrite (red) and axon (blue). (a), (b) Cases where axon response has higher amplitude compared to dendrite response(s); (c) case where axon response has lower amplitude compared to dendrite response(s); (d)  Response and raster plot of the soma of each neuron in a hippocampal neuron population.}
\label{fig:5}
\end{figure}
%\begin{figure}[ht!] 
%\begin{tabular}{c}
%        \subfigure[a]{
%            \includegraphics[width=0.5\columnwidth]{figures/figure5_new/fig_5a_left_new_1.eps}
%                  \includegraphics[width=0.5\columnwidth]{figures/figure5_new/fig_5a_right.eps}
%       \label{fig:5a}
%        }\\
%        \subfigure[b]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure5_new/fig_5b_left.eps}
%          \includegraphics[width=0.5\columnwidth]{figures/figure5_new/fig_5b_right.eps}
%           \label{fig:5b}
%       }\\
% \subfigure[c]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure5_new/fig_5c_left.eps}
%          \includegraphics[width=0.5\columnwidth]{figures/figure5_new/fig_5c_right.eps}
%           \label{fig:5c}
%}\\
% \subfigure[d]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure5_new/fig_5d.eps}
%\includegraphics[width=0.5\columnwidth]{figures/figure5_new/fig_5d.eps}
%           \label{fig:5d} 
%}
%
%\end{tabular}
%\caption{Calcium oscillation in a single neuron and neuron population and corresponding spike trains represented by raster lot: soma (green), dendrite (red) and axon (blue) (a), (b) higher amplitude axon response (c) lower amplitude axon response (d) Raster plot of soma region in a neuron population.}
%\label{fig:5}
%\end{figure}

%
%\begin{figure}[ht!] 
%     \begin{center}
%\begin{tabular}{cc} 
%        \subfigure[ ]{%
%            \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5a_left.eps}
%            %\includegraphics[width=\columnwidth]{figures/figure5_new/fig_5a.eps}
%
%\label{fig:5a}
%        } 
%         \subfigure[]{%
%           \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5a_right.eps}
%           \label{fig:5b}
%        }\\ 
%        \subfigure[ ]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5b_left.eps}
%           \label{fig:5c}
%       }
% \subfigure[ ]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5b_right.eps}
%           \label{fig:5d}
%}\\
% \subfigure[ ]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5c_left.eps}
%           \label{fig:5e}
%}
% \subfigure[ ]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5c_right.eps}
%           \label{fig:5f}
%}\\
% \subfigure[ ]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5d_left.eps}
%           \label{fig:5g}
%        }
%\subfigure[ ]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5d_right.eps}
%           \label{fig:5h}
%}
%\end{tabular}
%\end{center} 
%    \caption{Calcium oscillation in a single neuron and neuron population and corresponding spike trains represented by raster plot: soma (green), dendrite (red) and axon (blue) (a), (b) higher amplitude axon response (c) lower amplitude axon response (d) Raw plot and corresponding Raster plot of soma region in a neuron population.}
%   \label{fig:5}
%\end{figure}



==> figures/figure6/fig6.tex <==
\begin{figure}[t!] 
     \begin{center}
\begin{tabular}{cc} 
        \subfigure[ ]{%
            \includegraphics[width=0.22\columnwidth]{figures/figure6/fig_6a.eps}
                \label{fig:6a}
\label{fig:first}
        }  
         \subfigure[ ]{%
           \includegraphics[width=0.22\columnwidth]{figures/figure6/fig_6b.eps}
           \label{fig:6b}
        }
        \subfigure[ ]{%
         \includegraphics[width=0.22\columnwidth]{figures/figure6/fig_6c.eps}
           \label{fig:6c}
        }%
\subfigure[ ]{%
         \includegraphics[width=0.22\columnwidth]{figures/figure6/fig_6d.eps} 
           \label{fig:6d} 
        }%
\end{tabular}
\end{center} \vspace{-0.38cm}
    \caption{Simulation of intracellular calcium oscillation in hippocampal neurons. (a) and (b) Simulation of calcium spiking from proposed model and corresponding raster plot, (c) and (d) Experimental calcium spiking in a neuron population and corresponding raster plot.}
   \label{fig:6}
\end{figure}






%\begin{figure}[ht!] 
%\begin{tabular}{c}
%        \subfigure[]{
%            \includegraphics[width=0.5\columnwidth]{figures/figure6/fig_6a.eps}
%                  \includegraphics[width=0.5\columnwidth]{figures/figure6/fig_6b.eps}
%       \label{fig:5a}
%        }\\ 
%        \subfigure[]{%
%         \includegraphics[width=0.5\columnwidth]{figures/figure6/fig_6c.eps}
%          \includegraphics[width=0.5\columnwidth]{figures/figure6/fig_6d.eps}
%           \label{fig:5b}
%     }
%%\\ \vspace{-0.3cm}
%% \subfigure[]{%
%%         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5c_left.eps}
%%          \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5c_right.eps}
%%           \label{fig:5c}
%%}\\
%% \subfigure[]{%
%%         \includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5d_left.eps}
%%\includegraphics[width=0.5\columnwidth]{figures/figure5_1/fig_5d_right.eps}
%%           \label{fig:5d} 
%%}

%\end{tabular}
%\caption{Calcium oscillation in a single neuron and neuron population and corresponding spike trains represented by raster lot: soma (black), dendrite (red) and axon (blue) (a), (b) higher amplitude axon response (c) lower amplitude axon response (d)  Raw plot and corresponding Raster plot of soma region in a neuron population.}
%\label{fig:5}
%\end{figure}

%\begin{figure}[t!]
%\centering
%\includegraphics[width=\columnwidth]{figures/figure6/temp6.eps}
%\caption{Simulation of intracellular calcium oscillation in hippocampal neurons (a) and (b) Simulation of calcium spiking from proposed model and corresponding raster plot (c) and (d) Experimental calcium spiking in a neuron population and corresponding raster plot.}
%\label{fig:6}
%\end{figure}

%\begin{figure}[ht!] 
%     \begin{center}
%\begin{tabular}{cc} 
%        \subfigure[ ]{%
%           \includegraphics[width=0.22\columnwidth]{figures/figure6/fig_6a.eps}
%
%\label{fig:6a}
%        } 
%         \subfigure[]{%
%         \includegraphics[width=0.22\columnwidth]{figures/figure6/fig_6b.eps}
%           \label{fig:6b}
%        }
% \subfigure[ ]{%
%           \includegraphics[width=0.22\columnwidth]{figures/figure6/fig_6c.eps}       
%
%\label{fig:6c}
%        } 
%         \subfigure[]{%
%         \includegraphics[width=0.22\columnwidth]{figures/figure6/fig_6d.eps}
%           \label{fig:6d}
%        }
%\end{tabular}
%\end{center} 
% \caption{Simulation of intracellular calcium oscillation in hippocampal neurons (a) and (b) Simulation of calcium spiking from proposed model and corresponding raster plot (c) and (d) Experimental calcium spiking in a neuron population and corresponding raster plot.}
%   \label{fig:6}
%\end{figure}


%
%
%
%\begin{figure}[ht!] 
%     \begin{center}
%\begin{tabular}{cc} 
%        \subfigure[ ]{%
%           \includegraphics[width=0.25\columnwidth]{figures/figure6/untitled.png}
%            %\includegraphics[width=\columnwidth]{figures/figure5_new/fig_5a.eps}
%
%\label{fig:6a}
%        } 
%         \subfigure[]{%
%         \includegraphics[width=0.25\columnwidth]{figures/figure6/untitled.png}
%           \label{fig:6ab}
%        }
% \subfigure[ ]{%
%           \includegraphics[width=0.25\columnwidth]{figures/figure6/untitled.png}
%            %\includegraphics[width=\columnwidth]{figures/figure5_new/fig_5a.eps}
%
%\label{fig:6c}
%        } 
%         \subfigure[]{%
%         \includegraphics[width=0.22columnwidth]{figures/figure6/untitled.png}
%           \label{fig:5d}
%        }
%\end{tabular}
%\end{center} 
% \caption{Simulation of intracellular calcium oscillation in hippocampal neurons (a) and (b) Simulation of calcium spiking from proposed model and corresponding raster plot (c) and (d) Experimental calcium spiking in a neuron population and corresponding raster plot.}
%   \label{fig:6}
%\end{figure}



==> section/Spike_Train_Inference.tex <==
\section{Spike train inference}
\label{sec:append}
To infer spike train from time course of normalized fluorescence intensity, we used a fast nonnegative deconvolution algorithm assuming a linear relation between fluorescence intensity and calcium concentration subject to baseline offset and normal error. Specifically, we modeled the fluorescence measurement $F_t$ of any neuron (whose index $i$ is dropped for the sake of convenience) at time $t$ to be proportional to intracellular calcium concentration $C_t$:
%\begin{small}
\begin{equation}
F_t =\alpha C_{t} +\beta +\varepsilon_t,
\label{eq:1}
\end{equation} 
%\end{small} 
%\noindent 
where $\alpha$ denotes a sclae factor,  $\beta$  the baseline offset in calcium concentration of the cell, and the error $\varepsilon_{t} \sim iid ~N(0,\sigma^{2})$ at  time $t$ is zero mean Gaussian with standard deviation $\sigma$ and independently and identically distributed. Further,
the relation between calcium concentration at time $t$ and time $t-1$ is given by
%\begin{small}
\begin{equation}
C_t= (1-{\Delta}\mathbin{/}{\tau}) C_{t-1} + ({\Delta}\mathbin{/}{\tau}) C_{b}+ A n_t,
\label{eq:2}
\end{equation}
%\end{small}
where $\Delta$ is frame duration or 1/(frame rate) and associated number of spikes $n_t \sim iid \,\, Poisson ({\lambda} {\Delta})$ follows Poisson distribution with rate $\lambda$. The intracellular concentration raises by A $\mu$M for each spike and subsequently decays down to baseline concentration $C_b$ $\mu$M with time constant $\tau$.

Given the statistical model, the aim is to maximize posteriori probability of number of spikes $n_t$, given the fluorescence observations {\boldmath${F_t}$}:
%\begin{small}
\begin{equation}  
\hat{n} = \arg\max_{n_t \leq N_0 }  \ {{  \mbox {Pr} [n_t \vert F_t]}},
\label{eq:3}
\end{equation}
%\end{small}
where $N_0$ represents maximum possible number of spikes in a frame.
The inferred spiking rate vector $\hat{n}$ is thresholded for identifying the spikes. 

\textbf{Threshold selection}

In fast nonnegative deconvolution algorithm, the estimated spike rate indicate number of spikes at each time point. Unfortunately, such estimated spiking rates are generally noisy, and may lead to inference of erroneous spikes. We mitigated such errors in spike inference by setting an adaptive threshold on estimated spiking rate. Specifically, we chose the spiking threshold 
\begin{equation}  
P_{th} = 3 \sigma_p, 
\label{eq:threshold}
%\end{align}
\end{equation}
where $\sigma_p$ indicates standard deviation of inferred spiking rate vector $\hat{n}$. The instants where spiking rate is greater than spiking threshold, $P_{th}$ are set as binary one (high spiking) otherwise zero (low spiking). Such binary spike sequences used for further analysis.





==> section/ref.tex <==
\begin{thebibliography}{99}

\bibitem{c1} Y. Penn, M. Segal, and E. Moses, Network synchronization in hippocampal neurons, Proceedings of the National Academy of Sciences, Mar. 2016, 113(12), pp.3341-6.

\bibitem{c2} S. Zeng, B. Li, S. Zeng, S. Chen, Simulation of spontaneous Ca 2+ oscillations in astrocytes mediated by voltage-gated calcium channels, Biophysical journal, Nov. 2009, 97(9), pp.2429-37.
\bibitem{c3} M. Goldberg, M. De Pitta, V. Volman, H. Berry, E. Ben-Jacob, Nonlinear gap junctions enable long-distance propagation of pulsating calcium waves in astrocyte networks, PLoS Comput Biol,  Aug. 2010, 6(8), e1000909.
\bibitem{c4} D. J. O'Shea, E. Trautmann, C. Chandrasekaran, S. Stavisky , J. C. Kao, M. Sahani, S. Ryu, K. Deisseroth, K.V. Shenoy, The need for calcium imaging in nonhuman primates: New motor neuroscience and brain-machine interfaces, Exp Neurol, 2017, 287(Pt 4), pp. 437-451.
\bibitem{c5} J. Cichon, and W.B. Gan, Branch-specific dendritic Ca(2+) spikes cause persistent synaptic plasticity, Nature, 2015, 520(7546), pp.180-5.
\bibitem{c6} C. Y. Yang, A. J. Woolley, D. Tsai, G. J. Suaning, J. W. Morley, N. H. Lovell, Calcium Imaging of Retinal Ganglion Cell Dendritic Responses to Extracellular Microelectrode Stimulation, in 7th International IEEE/EMBS Conference on Neural Engineering (NER), Apr 2015, pp.438-441.
\bibitem{c7} M. Lavrentovich, S. Hemkin, A mathematical model of spontaneous calcium oscillations in astrocytes, J. Theoritical Biology, 2008, 251(4), pp.553-560.
\bibitem{c8}  S. Mennerick, and C. F. Zorumski, Presynaptic influence on the time course of fast excitatory synaptic currents in cultured hippocampal cells,The Journal of neuroscience,  Apr 1995, 15(4), pp.3178-92.
\bibitem{c9} L. Giri, A. K. Patel, W. A. Karunarathne, V. Kalyanaraman, K. V. Venkatesh, N. Gautam, A G-protein subunit translocation embedded network motif underlies GPCR regulation of calcium oscillations, Biophys J, 2014. 107(1), pp.242-54.
\bibitem{c10} J. T. Vogelstein,  A. M. Packer, T. A. Machado, T. Sippy, B. Babadi, R. Yuste, L. Paninski, Fast nonnegative deconvolution for spike train inference from population calcium imaging, Journal of neurophysiology, 2010, 104(6), pp.3691-3704.

\end{thebibliography}
